Benchmarking Actor-Critic Deep Reinforcement Learning Algorithms for Robotics Control with Action Constraints

This study presents a benchmark for evaluating action-constrained reinforcement learning (RL) algorithms. In action-constrained RL, each action taken by the learning system must comply with certain constraints. These constraints are crucial for ensuring the feasibility and safety of actions in real-world systems. We evaluate existing algorithms and their novel variants across multiple robotics control environments, encompassing multiple action constraint types. Our evaluation provides the first in-depth perspective of the field, revealing surprising insights, including the effectiveness of a straightforward baseline approach. The benchmark problems and associated code utilized in our experiments are made available online at github.com/omron-sinicx/action-constrained-RL-benchmark for further research and development.

==> reward_table.tex <==
\begin{table*}[t]
    \centering
    \begin{tabularx}{\textwidth}{ll|CCCCCCCCCCCCCC}
    \toprule[1pt]
%    & \multicolumn{6}{C}{\textbf{Algorithms}}\\
    &B.S.&D+CP&D+CP+P&D+P&D+P+P&D+OP&D+OP+P&NFW&ONFW&D+AP&D+RS&S+P&S+P+P&S+AP&S+RS\\
    \midrule
N&100& -5.54& - & - & - & - & - & -5.46&\textbf{-4.41}&-10.7&-5.48&\textbf{-4.39}&-&-4.86&\textbf{-4.47}\\
&&$\pm 0.16$& & & & & &$\pm 0.11$&$\pm 0.08$&$\pm 5.1$&$\pm 0.15$&$\pm 0.12$&&$\pm 0.15$&$\pm 0.12$\\
    \midrule
L2&100&-5.48&-5.36&-5.48&-5.17&-5.23&\textbf{-4.95}&-5.69&\textbf{-4.83}&-5.41&-5.24&-6.62&\textbf{-5.09}&-5.13&-6.85\\
&&$\pm 0.54$&$\pm 0.13$&$\pm 0.12$&$\pm 0.06$&$\pm 0.11$&$\pm 0.06$&$\pm 0.19$&$\pm 0.09$&$\pm 0.19$&$\pm 0.15$&$\pm 0.26$&$\pm 0.11$&$\pm 0.30$&$\pm 0.17$\\
    \midrule
         O03&100&-6.73&-5.79&-6.49&-5.91&-5.83&-5.85&-6.09&\textbf{-5.08}&-5.86&-5.78&-6.05&\textbf{-5.60}&\textbf{-5.20}&-10.3\\
&&$\pm 0.59$&$\pm 0.09$&$\pm 0.23$&$\pm 0.08$&$\pm 0.16$&$\pm 0.11$&$\pm 0.18$&$\pm 0.07$&$\pm 0.14$&$\pm 0.13$&$\pm 0.17$&$\pm 0.15$&$\pm 0.17$&$\pm 0.3$\\
    \midrule
         O10&100&-5.52&-4.95&-5.82&-5.22&-5.18&-5.13&-5.35&\textbf{-4.41}&-5.21&-5.35&-6.06&\textbf{-4.66}&\textbf{-4.51}&-4.85\\
&&$\pm 0.41$&$\pm 0.10$&$\pm 0.14$&$\pm 0.16$&$\pm 0.10$&$\pm 0.09$&$\pm 0.11$&$\pm 0.06$&$\pm 0.14$&$\pm 0.18$&$\pm 0.21$&$\pm 0.09$&$\pm 0.11$&$\pm 0.13$\\
    \midrule
         O30&100&-4.95&-5.13&-5.38&-5.06&-4.91&-4.90&-5.23&\textbf{-4.29}&-5.15&-5.24&-6.31&-4.75&\textbf{-4.53}&\textbf{-4.51}\\
&&$\pm 0.16$&$\pm 0.16$&$\pm 0.16$&$\pm 0.10$&$\pm 0.12$&$\pm 0.09$&$\pm 0.13$&$\pm 0.07$&$\pm 0.12$&$\pm 0.21$&$\pm 0.16$&$\pm 0.12$&$\pm 0.11$&$\pm 0.13$\\
    \midrule
         M&100&-9.90&-5.03&-6.63&-5.22&-5.02&-5.10&-5.60&\textbf{-4.57}&-4.94&-5.13&-5.01&-\textbf{4.57}&-4.60&\textbf{-4.46}\\
&&$\pm 0.57$&$\pm 0.09$&$\pm 0.19$&$\pm 0.12$&$\pm 0.11$&$\pm 0.13$&$\pm 0.17$&$\pm 0.06$&$\pm 0.15$&$\pm 0.14$&$\pm 0.14$&$\pm 0.10$&$\pm 0.11$&$\pm 0.13$\\
    \midrule
         H+M&16&862&1734&1635&4274&2593&3261&5603&6076&5676&4910&\textbf{7556}&\textbf{6754}&\textbf{6178}&5664\\
         &&$\pm 218$&$\pm 345$&$\pm 318$&$\pm 373$&$\pm 566$&$\pm 569$&$\pm 328$&$\pm 241$&$\pm 338$&$\pm 319$&$\pm 275$&$\pm 348$&$\pm 515$&$\pm 351$\\
    \cmidrule{2-16}
         &100&409&1995&4025&7223&-&-&6583&6220&7427&\textbf{8087}&\textbf{8074}&\textbf{8647}&5922&7606\\
&&$\pm 171$&$\pm 531$&$\pm 384$&$\pm 347$&&&$\pm 294$&$\pm 175$&$\pm 381$&$\pm 423$&$\pm 990$&$\pm 737$&$\pm 896$&$\pm 730$\\
    \midrule
         W+M&16&1373&934&1216&1331&651&838&2673&2434&3172&3009&\textbf{3299}&3248&\textbf{3307}&\textbf{3300}\\
&&$\pm 417$&$\pm 423$&$\pm 421$&$\pm 450$&$\pm 394$&$\pm 413$&$\pm 112$&$\pm 172$&$\pm 51$&$\pm 62$&$\pm 33$&$\pm 44$&$\pm 28$&$\pm 32$\\
    \cmidrule{2-16}
         &100&1498&1804&1847&1748&-&-&2406&2412&3157&3114&3226&\textbf{3299}&\textbf{3330}&\textbf{3372}\\
&&$\pm 404$&$\pm 454$&$\pm 473$&$\pm 445$&&&$\pm 210$&$\pm 107$&$\pm 74$&$\pm 80$&$\pm 93$&$\pm 59$&$\pm 31$&$\pm 24$\\
    \midrule
         HC+O&16&581&1205&1638&3012&1805&1638&1751&1330&3233&3021&\textbf{4328}&\textbf{4677}&\textbf{4077}&\textbf{4077}\\
&&$\pm 124$&$\pm 210$&$\pm 433$&$\pm 191$&$\pm 394$&$\pm 353$&$\pm 192$&$\pm 97$&$\pm 160$&$\pm 235$&$\pm 98$&$\pm 125$&$\pm 303$&$\pm 137$\\
    \cmidrule{2-16}
         &100&551&591&3181&3931&-&-&2182&1874&3242&3336&\textbf{4709}&\textbf{5024}&4384&\textbf{4632}\\
&&$\pm 100$&$\pm 85$&$\pm 522$&$\pm 224$&&&$\pm 183$&$\pm 140$&$\pm 296$&$\pm 283$&$\pm 109$&$\pm 100$&$\pm 214$&$\pm 201$\\
    \bottomrule[1pt]
    \end{tabularx}
    \caption{Average Rewards}
    \label{tab:rewards}
\end{table*}

